Lost in the Middle, and In-Between: Enhancing Language Models' Ability to Reason Over Long Contexts in Multi-Hop QA

Previous work finds that recent long-context language models fail to make equal use of information in the middle of their inputs, preferring pieces of information located at the tail ends which creates an undue bias in situations where we would like models to be equally capable of using different parts of the input. Thus far, the problem has mainly only been considered in settings with single pieces of critical information, leading us to question what happens when multiple necessary pieces of information are spread out over the inputs. Here, we demonstrate the effects of the "lost in the middle" problem in the multi-hop question answering setting -- in which multiple reasoning "hops" over disconnected documents are required -- and show that performance degrades not only with respect to the distance of information from the edges of the context, but also between pieces of information. Additionally, we experiment with means of alleviating the problem by reducing superfluous document contents through knowledge graph triple extraction and summarization, and prompting models to reason more thoroughly using chain-of-thought prompting.

==> gpt_results.tex <==
\begin{table*}[htbp]
\centering
\tiny
\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|c|}
\hline
Dataset (Closed-book Score) & Prompt & 1,2 & 5,6 & 10,11 & 15,16 & 19,20 & 1,5 & 5,10 & 10,15 & 15,20 \\ \hline
\multirow{6}{*}{Hotpot (40.64\%)} & standard & 76.72\% & 71.13\% & 71.40\% & 72.81\% & 73.89\% & 73.75\% & 69.97\% & 70.16\% & 71.13\% \\
& standard + CoT & 79.26\% & 73.91\% & 75.10\% & 75.61\% & 76.64\% & 77.48\% & 72.89\% & 71.78\% & 74.13\% \\
& kg & 56.09\% & 53.82\% & 53.61\% & 54.28\% & 57.52\% & 56.12\% & 51.96\% & 52.01\% & 54.63\% \\
& kg + CoT & 34.94\% & 28.03\% & 29.57\% & 29.92\% & 31.14\% & 31.60\% & 28.25\% & 28.54\% & 29.84\% \\
& summaries & 60.11\% & 59.52\% & 58.30\% & 59.79\% & 60.73\% & 59.90\% & 57.01\% & 56.36\% & 58.71\% \\
& summaries + CoT & 60.63\% & 61.09\% & 58.84\% & 59.79\% & 61.92\% & 61.27\% & 57.84\% & 57.41\% & 57.90\% \\ \hline

\multirow{1}{*}{ MuSiQue (14.39\%)} & \phantom{} & 1,2 & 5,6 & 10,11 & 15,16 & 19,20 & 1,5 & 5,10 & 10,15 & 15,20 \\ \hline

\multirow{6}{*}{2-hop} & standard & 56.23\% & 43.45\% & 41.21\% & 43.93\% & 52.72\% & 53.83\% & 40.89\% & 38.18\% & 45.21\% \\
& standard + CoT & 58.47\% & 48.24\% & 44.25\% & 46.96\% & 53.83\% & 55.43\% & 48.08\% & 44.25\% & 47.28\% \\
& kg & 34.66\% & 25.88\% & 28.27\% & 30.51\% & 33.87\% & 30.51\% & 25.88\% & 27.00\% & 27.96\% \\
& kg + CoT & 14.06\% & 7.67\% & 9.90\% & 9.11\% & 10.86\% & 12.14\% & 8.63\% & 9.11\% & 9.90\% \\
& summaries & 39.46\% & 36.10\% & 34.50\% & 35.46\% & 41.05\% & 39.78\% & 33.71\% & 31.95\% & 33.39\% \\
& summaries + CoT & 40.73\% & 38.02\% & 38.18\% & 38.02\% & 39.46\% & 42.81\% & 39.62\% & 33.55\% & 36.58\% \\ \hline

\multirow{1}{*}{}  &  & 1, 2, 3 & 5, 6, 7 & 10, 11, 12 & 15, 16, 17 & 18, 19,20 & 1, 5, 10 & 5, 10, 15 & 10, 15, 20 &  \\ \hline

\multirow{6}{*}{3-hop} & standard & 58.95\% & 43.68\% & 45.79\% & 45.26\% & 52.11\% & 49.47\% & 41.84\% & 43.95\% & - \\
& standard + CoT & 57.89\% & 47.89\% & 43.16\% & 46.84\% & 50.79\% & 51.32\% & 43.95\% & 44.21\% & - \\
& kg & 34.47\% & 26.32\% & 25.26\% & 26.58\% & 28.68\% & 28.68\% & 23.68\% & 24.47\% & - \\
& kg + CoT & 5.79\% & 3.68\% & 5.79\% & 5.79\% & 5.79\% & 5.53\% & 5.53\% & 4.47\% & - \\
& summaries & 39.47\% & 36.05\% & 36.32\% & 35.53\% & 37.63\% & 36.32\% & 31.84\% & 33.68\% & - \\
& summaries + CoT & 37.37\% & 33.95\% & 36.05\% & 33.68\% & 38.16\% & 35.79\% & 33.16\% & 36.05\% & - \\ \hline

\multirow{1}{*}{}  & \phantom{} & 1,2,3,4 & 5,6,7,8 & 10,11,12,13 & 15,16,17,18 & 17,18, 19,20 & 1,3,5,7 & 5,7,9,11 & 10,12,14,16 & 14,16,18,20 \\ \hline

\multirow{6}{*}{4-hop} & standard & 59.11\% & 42.86\% & 50.25\% & 51.72\% & 58.62\% & 59.61\% & 47.78\% & 41.87\% & 53.20\% \\
& standard + CoT & 56.16\% & 46.31\% & 49.75\% & 45.81\% & 52.71\% & 52.71\% & 44.83\% & 39.41\% & 48.28\% \\
& kg & 32.02\% & 25.12\% & 26.60\% & 23.65\% & 29.56\% & 31.53\% & 27.09\% & 26.11\% & 23.15\% \\
& kg + CoT & 3.94\% & 3.45\% & 5.91\% & 5.91\% & 5.91\% & 4.93\% & 5.91\% & 3.94\% & 5.91\% \\
& summaries & 30.54\% & 30.05\% & 29.56\% & 27.59\% & 27.09\% & 31.03\% & 28.57\% & 26.60\% & 31.53\% \\
& summaries + CoT & 32.51\% & 26.11\% & 28.08\% & 27.09\% & 27.59\% & 30.05\% & 28.57\% & 28.57\% & 26.60\% \\ \hline

\multirow{1}{*}{2Wiki (44.99\%)} &  & 1,2 & 5,6 & 10,11 & 15,16 & 19,20 & 1,5 & 5,10 & 10,15 & 15,20 \\ \hline

\multirow{6}{*}{2-hop} & standard & 65.83\% & 59.26\% & 57.96\% & 60.18\% & 63.06\% & 63.61\% & 57.76\% & 56.42\% & 59.67\% \\
& standard + CoT & 67.90\% & 64.75\% & 65.24\% & 65.32\% & 68.63\% & 67.01\% & 63.04\% & 62.43\% & 65.56\% \\
& kg & 41.00\% & 38.97\% & 38.11\% & 40.11\% & 42.58\% & 40.86\% & 37.57\% & 37.83\% & 40.37\% \\
& kg + CoT & 25.99\% & 24.08\% & 24.32\% & 24.46\% & 26.11\% & 25.05\% & 24.38\% & 23.77\% & 24.42\% \\
& summaries & 44.72\% & 41.69\% & 41.30\% & 42.46\% & 44.17\% & 42.85\% & 40.69\% & 39.62\% & 41.20\% \\
& summaries + CoT & 46.10\% & 44.86\% & 44.76\% & 44.39\% & 46.20\% & 45.98\% & 43.46\% & 43.19\% & 43.95\% \\ \hline

\multirow{1}{*}{}  & \phantom{} & 1,2,3,4 & 5,6,7,8 & 10,11,12,13 & 15,16,17,18 & 17,18, 19,20 & 1,3,5,7 & 5,7,9,11 & 10,12,14,16 & 14,16,18,20 \\ \hline

\multirow{6}{*}{4-hop} & standard & 91.29\% & 90.04\% & 90.12\% & 89.82\% & 89.60\% & 89.82\% & 88.65\% & 89.24\% & 89.60\% \\
& standard + CoT & 93.27\% & 92.24\% & 93.70\% & 92.24\% & 93.12\% & 93.05\% & 92.24\% & 92.31\% & 92.46\% \\
& kg & 83.09\% & 83.24\% & 82.43\% & 82.72\% & 84.41\% & 82.94\% & 82.28\% & 82.58\% & 83.46\% \\
& kg + CoT & 65.15\% & 67.20\% & 67.94\% & 64.28\% & 64.13\% & 66.62\% & 65.96\% & 65.81\% & 63.47\% \\
& summaries & 89.17\% & 88.07\% & 86.16\% & 88.80\% & 88.14\% & 88.73\% & 86.90\% & 86.68\% & 88.21\% \\
& summaries + CoT & 94.80\% & 92.31\% & 93.41\% & 93.92\% & 92.83\% & 94.22\% & 92.97\% & 93.41\% & 93.48\% \\ \hline

\end{tabular}
\caption{Full experimental results of gpt-3.5-turbo-1106. Percentages next to dataset names are the closed-book scores for the full set.}
\label{tab:gpt_results}
\end{table*}

==> llama_results.tex <==
\begin{table*}[htbp]
\centering
\tiny
\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|c|}
\hline
Dataset (Closed-book Score) & Prompt & 1,2 & 5,6 & 10,11 & 15,16 & 19,20 & 1,5 & 5,10 & 10,15 & 15,20 \\ \hline

\multirow{6}{*}{Hotpot (12.21\%)} & standard & 3.11\% & 0.97\% & 0.86\% & 0.95\% & 0.86\% & 1.67\% & 0.95\% & 0.70\% & 0.89\% \\
& standard + CoT & 0.59\% & 0.46\% & 0.46\% & 0.46\% & 0.51\% & 0.49\% & 0.65\% & 0.59\% & 0.46\% \\
& kg & 25.76\% & 8.78\% & 9.15\% & 8.48\% & 7.89\% & 16.47\% & 9.29\% & 8.61\% & 7.56\% \\
& kg + CoT & 1.16\% & 0.97\% & 1.03\% & 1.05\% & 0.81\% & 0.89\% & 1.08\% & 0.89\% & 1.08\% \\
& summaries & 20.09\% & 4.73\% & 3.75\% & 3.65\% & 3.46\% & 10.29\% & 4.24\% & 3.48\% & 3.54\% \\
& summaries + CoT & 0.14\% & 0.16\% & 0.11\% & 0.16\% & 0.51\% & 0.08\% & 0.11\% & 0.24\% & 0.19\% \\ \hline

\multirow{6}{*}{}Musique (0.74\%) &  & 1,2 & 5,6 & 10,11 & 15,16 & 19,20 & 1,5 & 5,10 & 10,15 & 15,20 \\ \hline
\multirow{6}{*}{2-hop} & standard & 1.92\% & 0.00\% & 0.16\% & 0.00\% & 0.00\% & 1.12\% & 0.00\% & 0.00\% & 0.00\% \\
& standard + CoT & 0.16\% & 0.16\% & 0.16\% & 0.16\% & 0.32\% & 0.16\% & 0.48\% & 0.32\% & 0.32\% \\
& kg & 16.93\% & 0.64\% & 1.12\% & 1.12\% & 0.80\% & 9.42\% & 0.64\% & 1.44\% & 1.12\% \\
& kg + CoT & 0.16\% & 0.00\% & 0.16\% & 0.16\% & 0.16\% & 0.16\% & 0.16\% & 0.16\% & 0.16\% \\
& summaries & 6.87\% & 0.64\% & 0.32\% & 0.16\% & 0.48\% & 3.35\% & 0.80\% & 0.48\% & 0.32\% \\
& summaries + CoT & 0.16\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.16\% \\ \hline

\multirow{6}{*}{} &  & 1,2,3 & 5,6,7 & 10,11,12 & 15,16,17 & 18,19,20 & 1,5,10 & 5,10,15 & 10,15,20 & \\ \hline
\multirow{6}{*}{3-hop} & standard & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & - \\
& standard + CoT & 0.00\% & 0.00\% & 0.26\% & 0.00\% & 0.00\% & 0.00\% & 0.26\% & 0.26\% & - \\
& kg & 0.00\% & 0.00\% & 0.00\% & 0.26\% & 0.26\% & 0.00\% & 0.00\% & 0.26\% & - \\
& kg + CoT & 0.26\% & 0.26\% & 0.26\% & 0.26\% & 0.00\% & 0.26\% & 0.26\% & 0.00\% & - \\
& summaries & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & - \\
& summaries + CoT & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.26\% & 0.00\% & 0.00\% & 0.00\% & - \\ \hline

\multirow{6}{*}{} &  & 1,2,3,4 & 5,6,7,8 & 10,11,12,13 & 15,16,17,18 & 17,18,19,20 & 1,3,5,7 & 5,7,9,11 & 10,12,14,16 & 14,16,18,20 \\ \hline
\multirow{6}{*}{4-hop} & standard & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\
& standard + CoT & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\
& kg & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\
& kg + CoT & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\
& summaries & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\
& summaries + CoT & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\ \hline

\multirow{6}{*}{}2wiki (31.65\%) &  & 1,2 & 5,6 & 10,11 & 15,16 & 19,20 & 1,5 & 5,10 & 10,15 & 15,20 \\ \hline
\multirow{6}{*}{2-hop} & standard & 27.29\% & 5.02\% & 3.15\% & 3.09\% & 2.54\% & 17.39\% & 4.65\% & 3.17\% & 2.82\% \\
& standard + CoT & 0.26\% & 0.10\% & 0.06\% & 0.24\% & 0.16\% & 0.22\% & 0.26\% & 0.16\% & 0.14\% \\
& kg & 25.58\% & 7.90\% & 6.32\% & 6.44\% & 6.20\% & 17.53\% & 7.86\% & 6.52\% & 6.12\% \\
& kg + CoT & 0.81\% & 0.77\% & 0.89\% & 1.00\% & 1.02\% & 1.00\% & 1.06\% & 1.02\% & 1.02\% \\
& summaries & 28.99\% & 12.37\% & 4.31\% & 4.06\% & 3.51\% & 20.85\% & 10.20\% & 4.02\% & 3.82\% \\
& summaries + CoT & 0.12\% & 0.10\% & 0.08\% & 0.06\% & 0.06\% & 0.06\% & 0.10\% & 0.10\% & 0.08\% \\ \hline

\multirow{6}{*}{} &  & 1,2,3,4 & 5,6,7,8 & 10,11,12,13 & 15,16,17,18 & 17,18,19,20 & 1,3,5,7 & 5,7,9,11 & 10,12,14,16 & 14,16,18,20 \\ \hline
\multirow{6}{*}{4-hop} & standard & 30.75\% & 8.35\% & 5.42\% & 4.54\% & 3.95\% & 24.30\% & 8.64\% & 5.34\% & 3.73\% \\
& standard + CoT & 0.51\% & 0.51\% & 0.51\% & 1.10\% & 0.73\% & 0.51\% & 0.51\% & 0.88\% & 0.73\% \\
& kg & 43.56\% & 19.25\% & 14.49\% & 14.71\% & 14.49\% & 34.99\% & 19.33\% & 14.20\% & 13.69\% \\
& kg + CoT & 2.56\% & 3.15\% & 2.12\% & 2.34\% & 2.34\% & 1.98\% & 2.64\% & 2.27\% & 2.42\% \\
& summaries & 56.95\% & 16.91\% & 5.93\% & 5.20\% & 4.03\% & 36.53\% & 14.86\% & 5.71\% & 4.47\% \\
& summaries + CoT & 0.12\% & 0.00\% & 0.00\% & 0.07\% & 0.07\% & 0.06\% & 0.00\% & 0.00\% & 0.00\% \\ \hline

\end{tabular}
\caption{Full experimental results of llama-2-7b-longlora-8k-ft. Percentages next to dataset names are the closed-book scores for the full set.}
\label{table:performance}
\end{table*}


==> mpt_results.tex <==
% \begin{table*}[htbp]
% \centering
% \tiny
% \begin{tabular}{|l|l|c|c|c|c|c|c|c|c|c|}
% \hline
% Dataset (Closed-book Score) & Prompt & 1, 2 & 5, 6 & 10, 11 & 15, 16 & 19, 20 & 1, 5 & 5, 10 & 10, 15 & 15, 20 \\ \hline
% \multirow{6}{*}{Hotpot (14.88\%)} & standard & 51.90\% & 45.13\% & 46.50\% & 49.50\% & 53.23\% & 41.61\% & 38.54\% & 41.48\% & 47.18\% \\
% & standard + CoT & 57.17\% & 48.88\% & 49.96\% & 54.04\% & 59.09\% & 48.96\% & 46.26\% & 50.36\% & 55.60\% \\
% & kg & 32.57\% & 29.65\% & 30.16\% & 31.73\% & 35.35\% & 29.73\% & 29.25\% & 29.79\% & 33.11\% \\
% & kg + CoT & 42.45\% & 37.32\% & 37.89\% & 41.43\% & 44.88\% & 37.43\% & 36.46\% & 38.51\% & 41.21\% \\
% & summaries & 43.64\% & 35.05\% & 33.19\% & 34.19\% & 37.19\% & 37.27\% & 32.87\% & 32.57\% & 35.13\% \\
% & summaries + CoT & 52.88\% & 45.83\% & 41.94\% & 43.05\% & 46.34\% & 43.13\% & 39.97\% & 41.16\% & 43.05\% \\ \hline

% \multirow{6}{*}{}Musique (3.64\%) &  & 1, 2 & 5, 6 & 10, 11 & 15, 16 & 19, 20 & 1, 5 & 5, 10 & 10, 15 & 15, 20 \\ \hline
%  \multirow{6}{*}{2-hop} & standard & 30.35\% & 18.85\% & 20.77\% & 26.52\% & 36.42\% & 24.92\% & 20.93\% & 22.20\% & 27.64\% \\
% & standard + CoT & 40.42\% & 31.31\% & 29.23\% & 35.78\% & 43.29\% & 30.83\% & 27.80\% & 32.27\% & 35.78\% \\
% & kg & 22.20\% & 19.65\% & 17.89\% & 22.20\% & 26.20\% & 19.33\% & 18.85\% & 17.57\% & 20.29\% \\
% & kg + CoT & 26.04\% & 21.25\% & 21.57\% & 27.16\% & 31.79\% & 19.97\% & 20.77\% & 22.84\% & 24.92\% \\
% & summaries & 32.91\% & 22.52\% & 18.37\% & 18.21\% & 23.16\% & 26.04\% & 19.49\% & 17.25\% & 18.37\% \\
% & summaries + CoT & 37.70\% & 27.32\% & 24.92\% & 25.88\% & 30.99\% & 30.03\% & 25.56\% & 24.44\% & 25.40\% \\ \hline

% \multirow{1}{*}{}  &  & 1, 2, 3 & 5, 6, 7 & 10, 11, 12 & 15, 16, 17 & 18, 19,20 & 1, 5, 10 & 5, 10, 15 & 10, 15, 20 &  \\ \hline
% \multirow{6}{*}{3-hop}& standard & 33.95\% & 25.53\% & 25.79\% & 31.84\% & 39.74\% & 28.16\% & 27.63\% & 31.58\% & - \\ 
% & standard + CoT & 37.89\% & 28.95\% & 34.47\% & 32.89\% & 43.16\% & 32.89\% & 31.84\% & 33.42\% & - \\ 
% & kg & 24.47\% & 18.95\% & 17.37\% & 17.11\% & 22.37\% & 20.26\% & 18.16\% & 18.95\% & - \\ 
% & kg + CoT & 22.89\% & 23.16\% & 23.95\% & 26.32\% & 31.05\% & 20.00\% & 20.79\% & 26.84\% & - \\ 
% & summaries & 38.95\% & 25.79\% & 20.26\% & 19.47\% & 20.53\% & 27.63\% & 20.00\% & 18.95\% & - \\ 
% & summaries + CoT & 35.00\% & 31.32\% & 28.95\% & 26.58\% & 30.79\% & 25.26\% & 26.05\% & 24.47\% & - \\ \hline

% \multirow{1}{*}{}  & \phantom{} & 1,2,3,4 & 5,6,7,8 & 10,11,12,13 & 15,16,17,18 & 17,18, 19,20 & 1,3,5,7 & 5,7,9,11 & 10,12,14,16 & 14,16,18,20 \\ \hline
% \multirow{6}{*}{4-hop} & standard & 23.15\% & 17.24\% & 17.24\% & 24.14\% & 23.15\% & 20.69\% & 17.73\% & 20.20\% & 21.67\% \\
% & standard + CoT & 28.57\% & 25.12\% & 25.12\% & 26.60\% & 37.44\% & 29.06\% & 25.62\% & 27.09\% & 37.93\% \\
% & kg & 33.00\% & 33.50\% & 31.53\% & 35.47\% & 39.41\% & 33.00\% & 28.08\% & 29.06\% & 35.47\% \\
% & kg + CoT & 33.50\% & 28.57\% & 35.47\% & 35.47\% & 46.80\% & 28.57\% & 27.59\% & 33.00\% & 40.89\% \\
% & summaries & 26.11\% & 10.84\% & 11.33\% & 9.85\% & 12.32\% & 19.70\% & 9.85\% & 10.34\% & 12.32\% \\
% & summaries + CoT & 27.09\% & 24.14\% & 18.23\% & 23.65\% & 24.63\% & 24.14\% & 22.66\% & 20.20\% & 19.70\% \\ \hline

% \multirow{1}{*}{}2wiki (20.13\%) &   & 1, 2 & 5, 6 & 10, 11 & 15, 16 & 19, 20 & 1, 5 & 5, 10 & 10, 15 & 15, 20 \\ \hline

% \multirow{6}{*}{2-hop} & standard & 33.81\% & 27.22\% & 27.10\% & 28.24\% & 31.65\% & 32.59\% & 27.33\% & 26.86\% & 28.79\% \\
% & standard + CoT & 42.42\% & 38.16\% & 37.22\% & 38.91\% & 42.95\% & 36.18\% & 35.31\% & 37.38\% & 39.54\% \\
% & kg & 24.77\% & 23.24\% & 22.47\% & 22.90\% & 24.18\% & 24.18\% & 22.86\% & 21.80\% & 23.41\% \\
% & kg + CoT & 33.54\% & 31.51\% & 30.13\% & 32.32\% & 33.93\% & 30.03\% & 29.87\% & 30.07\% & 32.36\% \\
% & summaries & 26.25\% & 23.47\% & 21.62\% & 22.19\% & 22.41\% & 25.05\% & 22.65\% & 21.90\% & 22.06\% \\
% & summaries + CoT & 34.82\% & 32.77\% & 29.80\% & 31.84\% & 32.63\% & 28.91\% & 29.68\% & 30.27\% & 31.25\% \\ \hline

% \multirow{1}{*}{}  & \phantom{} & 1,2,3,4 & 5,6,7,8 & 10,11,12,13 & 15,16,17,18 & 17,18, 19,20 & 1,3,5,7 & 5,7,9,11 & 10,12,14,16 & 14,16,18,20 \\ \hline
% \multirow{6}{*}{4-hop}& standard & 52.42\% & 51.39\% & 51.17\% & 51.46\% & 51.90\% & 51.68\% & 51.32\% & 50.73\% & 53.00\% \\
% & standard + CoT & 75.33\% & 72.91\% & 72.62\% & 74.45\% & 73.50\% & 73.72\% & 73.43\% & 73.06\% & 72.69\% \\
% & kg & 50.29\% & 52.34\% & 52.86\% & 50.15\% & 50.22\% & 50.22\% & 51.68\% & 52.20\% & 50.22\% \\
% & kg + CoT & 66.03\% & 65.96\% & 67.79\% & 63.91\% & 63.18\% & 67.86\% & 68.01\% & 65.01\% & 62.45\% \\
% & summaries & 54.10\% & 55.78\% & 51.54\% & 52.20\% & 53.44\% & 55.12\% & 54.54\% & 52.42\% & 54.47\% \\
% & summaries + CoT & 76.43\% & 74.16\% & 71.01\% & 72.40\% & 74.52\% & 72.47\% & 70.94\% & 71.38\% & 73.13\% \\ \hline
% \end{tabular}
% \caption{Full experimental results of gpt-3.5-turbo-1106.}
% \label{table:mpt7b8kinstruct}
% \end{table*}


\begin{table*}[htbp]
\centering
\tiny
\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|c|}
\hline
Dataset (Closed-book Score) & Prompt & 1,2 & 5,6 & 10,11 & 15,16 & 19,20 & 1,5 & 5,10 & 10,15 & 15,20 \\ \hline
\multirow{6}{*}{Hotpot (14.88\%)} & standard & 51.90\% & 45.13\% & 46.50\% & 49.50\% & 53.23\% & 41.61\% & 38.54\% & 41.48\% & 47.18\% \\
& standard + CoT & 57.17\% & 48.88\% & 49.96\% & 54.04\% & 59.09\% & 48.96\% & 46.26\% & 50.36\% & 55.60\% \\
& kg & 32.57\% & 29.65\% & 30.16\% & 31.73\% & 35.35\% & 29.73\% & 29.25\% & 29.79\% & 33.11\% \\
& kg + CoT & 42.45\% & 37.32\% & 37.89\% & 41.43\% & 44.88\% & 37.43\% & 36.46\% & 38.51\% & 41.21\% \\
& summaries & 43.64\% & 35.05\% & 33.19\% & 34.19\% & 37.19\% & 37.27\% & 32.87\% & 32.57\% & 35.13\% \\
& summaries + CoT & 52.88\% & 45.83\% & 41.94\% & 43.05\% & 46.34\% & 43.13\% & 39.97\% & 41.16\% & 43.05\% \\ \hline

\multirow{6}{*}{}Musique (3.64\%) &  & 1,2 & 5,6 & 10,11 & 15,16 & 19,20 & 1,5 & 5,10 & 10,15 & 15,20 \\ \hline
2-hop & standard & 30.35\% & 18.85\% & 20.77\% & 26.52\% & 36.42\% & 24.92\% & 20.93\% & 22.20\% & 27.64\% \\
& standard + CoT & 40.42\% & 31.31\% & 29.23\% & 35.78\% & 43.29\% & 30.83\% & 27.80\% & 32.27\% & 35.78\% \\
& kg & 22.20\% & 19.65\% & 17.89\% & 22.20\% & 26.20\% & 19.33\% & 18.85\% & 17.57\% & 20.29\% \\
& kg + CoT & 26.04\% & 21.25\% & 21.57\% & 27.16\% & 31.79\% & 19.97\% & 20.77\% & 22.84\% & 24.92\% \\
& summaries & 32.91\% & 22.52\% & 18.37\% & 18.21\% & 23.16\% & 26.04\% & 19.49\% & 17.25\% & 18.37\% \\
& summaries + CoT & 37.70\% & 27.32\% & 24.92\% & 25.88\% & 30.99\% & 30.03\% & 25.56\% & 24.44\% & 25.40\% \\ \hline

\multirow{1}{*}{}  &  & 1,2,3 & 5,6,7 & 10,11,12 & 15,16,17 & 18,19,20 & 1,5,10 & 5,10,15 & 10,15,20 &  \\ \hline

\multirow{6}{*}{3-hop} & standard & 33.95\% & 25.53\% & 25.79\% & 31.84\% & 39.74\% & 28.16\% & 27.63\% & 31.58\% & - \\ 
& standard + CoT & 37.89\% & 28.95\% & 34.47\% & 32.89\% & 43.16\% & 32.89\% & 31.84\% & 33.42\% & - \\ 
& kg & 24.47\% & 18.95\% & 17.37\% & 17.11\% & 22.37\% & 20.26\% & 18.16\% & 18.95\% & - \\ 
& kg + CoT & 22.89\% & 23.16\% & 23.95\% & 26.32\% & 31.05\% & 20.00\% & 20.79\% & 26.84\% & - \\ 
& summaries & 38.95\% & 25.79\% & 20.26\% & 19.47\% & 20.53\% & 27.63\% & 20.00\% & 18.95\% & - \\ 
& summaries + CoT & 35.00\% & 31.32\% & 28.95\% & 26.58\% & 30.79\% & 25.26\% & 26.05\% & 24.47\% & - \\ \hline

\multirow{1}{*}{}  &  & 1,2,3,4 & 5,6,7,8 & 10,11,12,13 & 15,16,17,18 & 17,18, 19,20 & 1,3,5,7 & 5,7,9,11 & 10,12,14,16 & 14,16,18,20 \\ \hline

\multirow{6}{*}{4-hop} & standard & 23.15\% & 17.24\% & 17.24\% & 24.14\% & 23.15\% & 20.69\% & 17.73\% & 20.20\% & 21.67\% \\
& standard + CoT & 28.57\% & 25.12\% & 25.12\% & 26.60\% & 37.44\% & 29.06\% & 25.62\% & 27.09\% & 37.93\% \\
& kg & 33.00\% & 33.50\% & 31.53\% & 35.47\% & 39.41\% & 33.00\% & 28.08\% & 29.06\% & 35.47\% \\
& kg + CoT & 33.50\% & 28.57\% & 35.47\% & 35.47\% & 46.80\% & 28.57\% & 27.59\% & 33.00\% & 40.89\% \\
& summaries & 26.11\% & 10.84\% & 11.33\% & 9.85\% & 12.32\% & 19.70\% & 9.85\% & 10.34\% & 12.32\% \\
& summaries + CoT & 27.09\% & 24.14\% & 18.23\% & 23.65\% & 24.63\% & 24.14\% & 22.66\% & 20.20\% & 19.70\% \\ \hline

\multirow{1}{*}{2wiki (20.13\%)} &  & 1,2 & 5,6 & 10,11 & 15,16 & 19,20 & 1,5 & 5,10 & 10,15 & 15,20 \\ \hline
\multirow{6}{*}{2-hop} & standard & 33.81\% & 27.22\% & 27.10\% & 28.24\% & 31.65\% & 32.59\% & 27.33\% & 26.86\% & 28.79\% \\
& standard + CoT & 42.42\% & 38.16\% & 37.22\% & 38.91\% & 42.95\% & 36.18\% & 35.31\% & 37.38\% & 39.54\% \\
& kg & 24.77\% & 23.24\% & 22.47\% & 22.90\% & 24.18\% & 24.18\% & 22.86\% & 21.80\% & 23.41\% \\
& kg + CoT & 33.54\% & 31.51\% & 30.13\% & 32.32\% & 33.93\% & 30.03\% & 29.87\% & 30.07\% & 32.36\% \\
& summaries & 26.25\% & 23.47\% & 21.62\% & 22.19\% & 22.41\% & 25.05\% & 22.65\% & 21.90\% & 22.06\% \\
& summaries + CoT & 34.82\% & 32.77\% & 29.80\% & 31.84\% & 32.63\% & 28.91\% & 29.68\% & 30.27\% & 31.25\% \\ \hline

\multirow{1}{*}{} &  & 1,2,3,4 & 5,6,7,8 & 10,11,12,13 & 15,16,17,18 & 17,18, 19,20 & 1,3,5,7 & 5,7,9,11 & 10,12,14,16 & 14,16,18,20 \\ \hline

\multirow{6}{*}{4-hop} & standard & 52.42\% & 51.39\% & 51.17\% & 51.46\% & 51.90\% & 51.68\% & 51.32\% & 50.73\% & 53.00\% \\
& standard + CoT & 75.33\% & 72.91\% & 72.62\% & 74.45\% & 73.50\% & 73.72\% & 73.43\% & 73.06\% & 72.69\% \\
& kg & 50.29\% & 52.34\% & 52.86\% & 50.15\% & 50.22\% & 50.22\% & 51.68\% & 52.20\% & 50.22\% \\
& kg + CoT & 66.03\% & 65.96\% & 67.79\% & 63.91\% & 63.18\% & 67.86\% & 68.01\% & 65.01\% & 62.45\% \\
& summaries & 54.10\% & 55.78\% & 51.54\% & 52.20\% & 53.44\% & 55.12\% & 54.54\% & 52.42\% & 54.47\% \\
& summaries + CoT & 76.43\% & 74.16\% & 71.01\% & 72.40\% & 74.52\% & 72.47\% & 70.94\% & 71.38\% & 73.13\% \\ \hline
\end{tabular}
\caption{Full experimental results of mpt-7b-8k-instruct. Percentages next to dataset names are the closed-book scores for the full set.}
\label{table:mpt_results}
\end{table*}
